Generating Adversarial Examples with Graph Neural Networks

Recent years have witnessed the deployment of adversarial attacks to evaluate the robustness of Neural Networks. Past work in this field has relied on traditional optimization algorithms that ignore the inherent structure of the problem and data, or generative methods that rely purely on learning and often fail to generate adversarial examples where they are hard to find. To alleviate these deficiencies, we propose a novel attack based on a graph neural network (GNN) that takes advantage of the strengths of both approaches; we call it AdvGNN. Our GNN architecture closely resembles the network we wish to attack. During inference, we perform forward-backward passes through the GNN layers to guide an iterative procedure towards adversarial examples. During training, its parameters are estimated via a loss function that encourages the efficient computation of adversarial examples over a time horizon. We show that our method beats state-of-the-art adversarial attacks, including PGD-attack, MI-FGSM, and Carlini and Wagner attack, reducing the time required to generate adversarial examples with small perturbation norms by over 65\%. Moreover, AdvGNN achieves good generalization performance on unseen networks. Finally, we provide a new challenging dataset specifically designed to allow for a more illustrative comparison of adversarial attacks.

==> Tables/Hparams/mi-fgsm_hparam_round1.tex <==
\begin{tabular}{llllrrrrr}
\toprule
Steps &    lr &    mu & number\_props &  average\_time &  percentage\_timeout &  rank\_time &  rank\_timeout &  average\_rank \\
\midrule
  100 &   5.0 &   0.5 &           51 &     13.482818 &            0.039216 &        3.0 &           2.0 &          2.50 \\
  100 &   5.0 &  0.25 &           51 &     11.807226 &            0.058824 &        1.0 &           4.5 &          2.75 \\
  100 &   2.5 &   0.5 &           51 &     14.584559 &            0.039216 &        4.0 &           2.0 &          3.00 \\
  250 &  10.0 &   0.5 &           51 &     15.330973 &            0.039216 &        6.0 &           2.0 &          4.00 \\
  250 &  10.0 &  0.25 &           51 &     13.198162 &            0.078431 &        2.0 &           6.0 &          4.00 \\
  250 &   5.0 &  0.25 &           51 &     15.120650 &            0.058824 &        5.0 &           4.5 &          4.75 \\
  100 &   2.5 &  0.25 &           51 &     18.961278 &            0.098039 &        7.0 &           8.0 &          7.50 \\
  250 &   5.0 &   0.5 &           51 &     19.622577 &            0.098039 &        8.0 &           8.0 &          8.00 \\
  250 &   2.5 &  0.25 &           51 &     22.847611 &            0.098039 &       10.0 &           8.0 &          9.00 \\
  100 &  10.0 &   0.5 &           51 &     20.661144 &            0.117647 &        9.0 &          10.0 &          9.50 \\
  100 &  10.0 &  0.25 &           51 &     29.181259 &            0.196078 &       11.0 &          12.5 &         11.75 \\
  250 &   2.5 &   0.5 &           51 &     30.298572 &            0.176471 &       13.0 &          11.0 &         12.00 \\
  100 &   1.0 &  0.25 &           51 &     30.067365 &            0.196078 &       12.0 &          12.5 &         12.25 \\
   50 &  10.0 &   1.0 &            8 &     35.574486 &            0.250000 &       16.0 &          14.0 &         15.00 \\
  100 &   2.5 &   1.0 &           51 &     35.919374 &            0.254902 &       17.0 &          15.0 &         16.00 \\
  100 &   5.0 &   1.0 &           51 &     36.528986 &            0.274510 &       18.0 &          16.5 &         17.25 \\
  250 &   1.0 &  0.25 &           51 &     34.455830 &            0.313725 &       14.0 &          21.0 &         17.50 \\
  250 &  10.0 &   1.0 &           51 &     37.012438 &            0.274510 &       19.0 &          16.5 &         17.75 \\
  100 &   1.0 &   0.5 &           51 &     35.236049 &            0.313725 &       15.0 &          21.0 &         18.00 \\
  250 &   1.0 &   0.5 &           51 &     37.546140 &            0.294118 &       20.0 &          18.5 &         19.25 \\
  100 &  10.0 &   1.0 &           51 &     38.325157 &            0.313725 &       21.0 &          21.0 &         21.00 \\
   50 &  10.0 &   0.5 &           51 &     45.763461 &            0.294118 &       26.0 &          18.5 &         22.25 \\
  100 &   1.0 &   1.0 &           51 &     39.310409 &            0.352941 &       22.0 &          24.0 &         23.00 \\
  250 &   2.5 &   1.0 &           51 &     42.362907 &            0.352941 &       23.0 &          24.0 &         23.50 \\
  250 &   5.0 &   1.0 &           51 &     45.733445 &            0.352941 &       25.0 &          24.0 &         24.50 \\
  250 &   1.0 &   1.0 &           51 &     43.061304 &            0.392157 &       24.0 &          26.0 &         25.00 \\
   50 &  10.0 &  0.25 &           51 &     61.827208 &            0.529412 &       27.0 &          27.0 &         27.00 \\
\bottomrule
\end{tabular}

==> Tables/Hparams/mi-fgsm_hparam_round2.tex <==
\begin{tabular}{lllrrrrr}
\toprule
Steps &    lr &   mu &  average\_time &  percentage\_timeout &  rank\_time &  rank\_timeout &  average\_rank \\
\midrule
  100 &   5.0 &  0.3 &     10.257855 &                0.02 &        1.0 &           2.0 &          1.50 \\
  100 &   7.5 &  0.4 &     11.642885 &                0.02 &        2.0 &           2.0 &          2.00 \\
  100 &   7.5 &  0.3 &     11.965179 &                0.02 &        4.0 &           2.0 &          3.00 \\
  100 &   5.0 &  0.4 &     11.655632 &                0.04 &        3.0 &           5.0 &          4.00 \\
  200 &  10.0 &  0.4 &     11.976870 &                0.06 &        5.0 &           8.0 &          6.50 \\
  200 &   7.5 &  0.4 &     13.720857 &                0.04 &        9.0 &           5.0 &          7.00 \\
  100 &   7.5 &  0.5 &     13.417719 &                0.06 &        7.0 &           8.0 &          7.50 \\
  100 &   5.0 &  0.5 &     14.516541 &                0.04 &       11.0 &           5.0 &          8.00 \\
  200 &   7.5 &  0.3 &     13.049936 &                0.08 &        6.0 &          13.5 &          9.75 \\
  100 &   5.0 &  0.6 &     17.041385 &                0.06 &       13.0 &           8.0 &         10.50 \\
  200 &  10.0 &  0.3 &     13.465613 &                0.08 &        8.0 &          13.5 &         10.75 \\
  200 &   5.0 &  0.3 &     14.249055 &                0.08 &       10.0 &          13.5 &         11.75 \\
  200 &   5.0 &  0.5 &     17.407682 &                0.08 &       14.0 &          13.5 &         13.75 \\
  200 &  10.0 &  0.6 &     18.253074 &                0.08 &       15.0 &          13.5 &         14.25 \\
  200 &  10.0 &  0.5 &     18.395693 &                0.08 &       16.0 &          13.5 &         14.75 \\
  200 &   7.5 &  0.5 &     18.423255 &                0.08 &       17.0 &          13.5 &         15.25 \\
  100 &   7.5 &  0.6 &     17.022754 &                0.10 &       12.0 &          19.5 &         15.75 \\
  100 &  10.0 &  0.4 &     19.234430 &                0.08 &       19.0 &          13.5 &         16.25 \\
  200 &   5.0 &  0.4 &     19.152746 &                0.10 &       18.0 &          19.5 &         18.75 \\
  100 &  10.0 &  0.6 &     19.846970 &                0.10 &       20.0 &          19.5 &         19.75 \\
  200 &   7.5 &  0.6 &     24.215175 &                0.10 &       22.0 &          19.5 &         20.75 \\
  100 &  10.0 &  0.5 &     20.504655 &                0.12 &       21.0 &          22.0 &         21.50 \\
  100 &  10.0 &  0.3 &     24.331758 &                0.14 &       23.0 &          23.5 &         23.25 \\
  200 &   5.0 &  0.6 &     24.925002 &                0.14 &       24.0 &          23.5 &         23.75 \\
\bottomrule
\end{tabular}

==> Tables/adv_model.tex <==

% \subsection{Tables in process}
%  \sisetup{detect-weight=true,detect-inline-weight=math,detect-mode=true}
\begin{table*}[h]

%% local settings
\sisetup{detect-weight,mode=text}
% for avoiding siunitx using bold extended
\renewrobustcmd{\bfseries}{\fontseries{b}\selectfont}
\renewrobustcmd{\boldmath}{}
% abbreviation
\newrobustcmd{\B}{\bfseries}

	\centering
	\scriptsize
	\setlength{\tabcolsep}{4pt}
	\aboverulesep = 0.1mm  % 0.605mm
	\belowrulesep = 0.2mm  % 0.984mm

    
	\begin{adjustbox}{center}

\begin{tabular}{llrrrrrr}
% 			& & \multicolumn{2}{ c }{\Base-Easy}\\
			\toprule

% \toprule
     Method &    Seed    & Time(s) &  Timeout(\%) \\

    % \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-4}
    
\midrule
 PGD Attack &  2222 &   16.922 &  79.2  \\
 PGD Attack &  3333 &   16.222 &  78.2  \\
 PGD Attack &  4444 &   16.382 &  77.2 \\
    MI-FGSM+ &  2222 &    5.771 &  27.8    \\
    MI-FGSM+ &  3333 &     5.773  &  18.8 \\
    MI-FGSM+ &  4444 &    5.847 &  20.8  \\
     AdvGNN &  2222 &    4.079 &  12.9   \\
     AdvGNN &  3333 &    3.739  & 12.9  \\
     AdvGNN &  4444 &    3.851 &  14.9 \\
\bottomrule
\end{tabular}

	\end{adjustbox}
	\caption{\small We compare average (mean) solving time and the percentage of properties that the methods time out on when using a cut-off time of 100s and the random Pytorch seeds specified. The best performing method for each subcategory is highlighted in bold.}
	\label{table:adv_model}
\end{table*}

==> Tables/easy_exp_combined.tex <==

% \subsection{Tables in process}
%  \sisetup{detect-weight=true,detect-inline-weight=math,detect-mode=true}
\begin{table*}[h]

%% local settings
\sisetup{detect-weight,mode=text}
% for avoiding siunitx using bold extended
\renewrobustcmd{\bfseries}{\fontseries{b}\selectfont}
\renewrobustcmd{\boldmath}{}
% abbreviation
\newrobustcmd{\B}{\bfseries}

	\centering
	\scriptsize
	\setlength{\tabcolsep}{4pt}
	\aboverulesep = 0.1mm  % 0.605mm
	\belowrulesep = 0.2mm  % 0.984mm
	
	% bold elements in table
	%\renewrobustcmd{\bfseries}{\fontseries{b}\selectfont}
    %\renewrobustcmd{\boldmath}{}
    %\newrobustcmd{\B}{\bfseries}
    
	\begin{adjustbox}{center}

\begin{tabular}{lrrrrrr}
			& \multicolumn{2}{ c }{\Base-Easy} & \multicolumn{2}{ c }{\Wide-Easy} & \multicolumn{2}{ c }{\Deep-Easy} \\
			\toprule

% \toprule
     Method &    Time(s) &  Timeout(\%) &  Time(s) &  Timeout(\%) &  Time(s) &  Timeout(\%) \\

    \cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
    
% \midrule
%      AdvGNN &    0.521 &       0.000 &         0.856 &             0.33 &         2.082 &            0.667 \\
%     MI-FGSM &    2.262 &       0.520 &         1.139 &             0.33 &         2.596 &            0.800 \\
%  PGD Attack &   12.389 &       7.124 &         5.632 &             2.42 &         8.245 &            3.200 \\
 PGD Attack &   12.430 &       7.124 &         5.647 &            2.420 &         8.265 &            3.200 \\
 MI-FGSM+ &    2.266 &       0.520 &         1.142 &            \B0.330 &         2.603 &            0.800 \\
 C\&W &   67.500 &      62.402 &        57.170 &           50.495 &        72.356 &           67.600 \\
 AdvGNN &    \B0.521 &       \B0.000 &         \B0.859 &            \B0.330 &         \B2.087 &            \B0.667 \\



\bottomrule
\end{tabular}

	\end{adjustbox}
	\caption{\small We compare average (mean) solving time and the percentage of properties that the methods time out on when using a cut-off time of 100s. The best performing method for each subcategory is highlighted in bold.}
	\label{table:easy_combined}
\end{table*}

==> Tables/easy_exp_seeds.tex <==

% \subsection{Tables in process}
%  \sisetup{detect-weight=true,detect-inline-weight=math,detect-mode=true}
\begin{table*}[h]

%% local settings
\sisetup{detect-weight,mode=text}
% for avoiding siunitx using bold extended
\renewrobustcmd{\bfseries}{\fontseries{b}\selectfont}
\renewrobustcmd{\boldmath}{}
% abbreviation
\newrobustcmd{\B}{\bfseries}

	\centering
	\scriptsize
	\setlength{\tabcolsep}{4pt}
	\aboverulesep = 0.1mm  % 0.605mm
	\belowrulesep = 0.2mm  % 0.984mm
	
	% bold elements in table
	%\renewrobustcmd{\bfseries}{\fontseries{b}\selectfont}
    %\renewrobustcmd{\boldmath}{}
    %\newrobustcmd{\B}{\bfseries}
    
	\begin{adjustbox}{center}

\begin{tabular}{llrrrrrr}
			& & \multicolumn{2}{ c }{\Base-Easy} & \multicolumn{2}{ c }{\Wide-Easy} & \multicolumn{2}{ c }{\Deep-Easy} \\
			\toprule

% \toprule
     Method &    Seed    & Time(s) &  Timeout(\%) &  Time(s) &  Timeout(\%) &  Time(s) &  Timeout(\%) \\

    \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}
    
% \midrule
 PGD Attack &  2222 &   12.765 &       6.864 &         5.783 &             2.64 &         8.842 &              4.0 \\
 PGD Attack &  3333 &   12.053 &       7.176 &         4.723 &             2.64 &         7.410 &              2.8 \\
 PGD Attack &  4444 &   12.349 &       7.332 &         6.389 &             1.98 &         8.483 &              2.8 \\
    MI-FGSM+ &  2222 &    1.994 &       0.624 &         1.394 &             0.66 &         2.879 &              0.8 \\
    MI-FGSM+ &  3333 &    2.565 &       0.468 &         0.981 &             0.33 &         2.636 &              1.2 \\
    MI-FGSM+ &  4444 &    2.227 &       0.468 &         1.042 &             0.00 &         2.273 &              0.4 \\
    C\&W &     - &   67.500 &      62.402 &        57.170 &           50.495 &        72.356 &             67.6 \\
     AdvGNN &  2222 &    0.519 &       0.000 &         0.811 &             0.33 &         2.077 &              0.8 \\
     AdvGNN &  3333 &    0.505 &       0.000 &         0.830 &             0.33 &         1.985 &              0.8 \\
     AdvGNN &  4444 &    0.538 &       0.000 &         0.926 &             0.33 &         2.184 &              0.4 \\
\bottomrule
\end{tabular}

	\end{adjustbox}
	\caption{\small We compare average (mean) solving time and the percentage of properties that the methods time out on when using a cut-off time of 100s and the random Pytorch seeds specified. The best performing method for each subcategory is highlighted in bold.}
	\label{table:easy_seeds}
\end{table*}

==> Tables/main_exp_combined.tex <==

% \subsection{Tables in process}
%  \sisetup{detect-weight=true,detect-inline-weight=math,detect-mode=true}
\begin{table}[h]

%% local settings
\sisetup{detect-weight,mode=text}
% for avoiding siunitx using bold extended
\renewrobustcmd{\bfseries}{\fontseries{b}\selectfont}
\renewrobustcmd{\boldmath}{}
% abbreviation
\newrobustcmd{\B}{\bfseries}

	\centering
	\scriptsize
	\setlength{\tabcolsep}{4pt}
	\aboverulesep = 0.1mm  % 0.605mm
	\belowrulesep = 0.2mm  % 0.984mm
	
	% bold elements in table
	%\renewrobustcmd{\bfseries}{\fontseries{b}\selectfont}
    %\renewrobustcmd{\boldmath}{}
    %\newrobustcmd{\B}{\bfseries}
    
	\begin{adjustbox}{center}

\begin{tabular}{lrrrrrr}
			& \multicolumn{2}{ c }{Base} & \multicolumn{2}{ c }{Wide} & \multicolumn{2}{ c }{Deep} \\
			\toprule

% \toprule
     Method &    Time(s) &  Timeout(\%) &  Time(s) &  Timeout(\%) &  Time(s) &  Timeout(\%) \\

    \cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
    
% \midrule
%      AdvGNN &    0.521 &       0.000 &         0.856 &             0.33 &         2.082 &            0.667 \\
%     MI-FGSM &    2.262 &       0.520 &         1.139 &             0.33 &         2.596 &            0.800 \\
%  PGD Attack &   12.389 &       7.124 &         5.632 &             2.42 &         8.245 &            3.200 \\
%  PGD Attack &   X &       X &         X &            X &         X &            X \\
%  MI-FGSM &    X &       X &         X &            X &         X &            X \\
%  C\&W &   X &      X &        X &           X &        X &           X \\
%  AdvGNN &    X &       X &         X &            X &         X &            X \\

%  PGD Attack &   87.354 &      82.995 &        80.542 &           74.917 &        83.764 &             79.2 \\
%  MI-FGSM &   39.897 &      26.677 &        31.583 &           21.122 &        \B59.887 &             \B46.4 \\
%  AdvGNN &   \B14.152 &      \B10.296 &        \B24.429 &           \B18.812 &        61.787 &             54.0 \\
         

 PGD Attack &   87.375 &      83.073 &        80.421 &           75.413 &        84.347 &           80.200 \\ 
 MI-FGSM+ &   40.438 &      27.145 &        31.144 &           20.462 &        \B60.578 &           \B47.867 \\
 C\&W &   97.385 &      95.164 &        96.366 &           93.729 &        99.321 &           97.600 \\
 AdvGNN &   \B13.527 &       \B9.412 &        \B24.089 &           \B18.482 &        61.703 &           54.133 \\
       
\bottomrule
\end{tabular}

	\end{adjustbox}
	\caption{\small We compare average (mean) solving time and the percentage of properties that the methods time out on when using a cut-off time of 100s. The best performing method for each subcategory is highlighted in bold.}
	\label{table:main_combined}
\end{table}

==> Tables/old/Base_Wide_Deep.tex <==

% \subsection{Tables in process}
%  \sisetup{detect-weight=true,detect-inline-weight=math,detect-mode=true}
\begin{table*}[]

%% local settings
\sisetup{detect-weight,mode=text}
% for avoiding siunitx using bold extended
\renewrobustcmd{\bfseries}{\fontseries{b}\selectfont}
\renewrobustcmd{\boldmath}{}
% abbreviation
\newrobustcmd{\B}{\bfseries}

	\centering
	\scriptsize
	\setlength{\tabcolsep}{4pt}
	\aboverulesep = 0.1mm  % 0.605mm
	\belowrulesep = 0.2mm  % 0.984mm
	
	% bold elements in table
	%\renewrobustcmd{\bfseries}{\fontseries{b}\selectfont}
    %\renewrobustcmd{\boldmath}{}
    %\newrobustcmd{\B}{\bfseries}
    
	\begin{adjustbox}{center}
		\begin{tabular}{
				l
				S[table-format=4.3]
				S[table-format=4.3]
				S[table-format=4.3]
				S[table-format=4.3]
				S[table-format=4.3]
				S[table-format=4.3]
				S[table-format=4.3]
				S[table-format=4.3]
				S[table-format=4.3]
			}
			& \multicolumn{2}{ c }{Base} & \multicolumn{2}{ c }{Wide} & \multicolumn{2}{ c }{Deep} \\
			\toprule
			
			\multicolumn{1}{ c }{Method} &
			\multicolumn{1}{ c }{time(s)} &
			\multicolumn{1}{ c }{$\%$Timeout} &
			\multicolumn{1}{ c }{time(s)} &
			\multicolumn{1}{ c }{$\%$Timeout} &
			\multicolumn{1}{ c }{time(s)} &
			\multicolumn{1}{ c }{$\%$Timeout} \\
			
			\cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
			

			
			\multicolumn{1}{ c }{\textsc{PGD}}
			& X
			& X
			
			& X
			& X
			
			& X
			& X\\
			
			\multicolumn{1}{ c }{\textsc{MI-FGSM}}
			& X
			& X
			
			& X
			& X
			
			& X
			& X\\
			
			\multicolumn{1}{ c }{\textsc{CW}}
			& X
			& X
			
			& X
			& X
			
			& X
			& X\\
			
			\multicolumn{1}{ c }{\textsc{AdvGNN}}
			& X
			& X
			
			& X
			& X
			
			& X
			& X\\
			
			\bottomrule
			
		\end{tabular}
	\end{adjustbox}
	\caption{\small We compare average (mean) solving time, average number of subdomains solved, and the percentage of properties that the methods time out on when using a cut-off time of 100s. The best performing method for each subcategory is highlighted in bold.}
	\label{table:base_wide_deep}
\end{table*}

==> Tables/old/base.tex <==

% \subsection{Tables in process}
%  \sisetup{detect-weight=true,detect-inline-weight=math,detect-mode=true}
\begin{table}

%% local settings
\sisetup{detect-weight,mode=text}
% for avoiding siunitx using bold extended
\renewrobustcmd{\bfseries}{\fontseries{b}\selectfont}
\renewrobustcmd{\boldmath}{}
% abbreviation
\newrobustcmd{\B}{\bfseries}

	\scriptsize
	\setlength{\tabcolsep}{4pt}
	\aboverulesep = 0.1mm  % 0.605mm
	\belowrulesep = 0.2mm  % 0.984mm
	
	% bold elements in table
	%\renewrobustcmd{\bfseries}{\fontseries{b}\selectfont}
    %\renewrobustcmd{\boldmath}{}
    %\newrobustcmd{\B}{\bfseries}
    
	\begin{adjustbox}{center}

\begin{tabular}{lrr}
			& \multicolumn{2}{ c }{Base} \\
			\toprule

% \toprule
     Method &    Time(s) &  Timeout(\%) \\

    \cmidrule(lr){1-1} \cmidrule(lr){2-3}
    
% \midrule
%      AdvGNN &    0.521 &       0.000 &         0.856 &             0.33 &         2.082 &            0.667 \\
%     MI-FGSM &    2.262 &       0.520 &         1.139 &             0.33 &         2.596 &            0.800 \\
%  PGD Attack &   12.389 &       7.124 &         5.632 &             2.42 &         8.245 &            3.200 \\
%  PGD Attack &   X &       X &         X &            X &         X &            X \\
%  MI-FGSM &    X &       X &         X &            X &         X &            X \\
%  C\&W &   X &      X &        X &           X &        X &           X \\
%  AdvGNN &    X &       X &         X &            X &         X &            X \\

%  PGD Attack &   87.354 &      82.995 &        80.542 &           74.917 &        83.764 &             79.2 \\
%  MI-FGSM &   39.897 &      26.677 &        31.583 &           21.122 &        \B59.887 &             \B46.4 \\
%  AdvGNN &   \B14.152 &      \B10.296 &        \B24.429 &           \B18.812 &        61.787 &             54.0 \\
         

 PGD Attack &   87.375 &      83.073        \\ 
 MI-FGSM &   40.438 &      27.145     \\
 C\&W &   97.385 &      95.164 \\
 AdvGNN &   \B13.527 &       \B9.412   \\
       
\bottomrule
\end{tabular}

	\end{adjustbox}
	\caption{\small We compare average (mean) solving time and the percentage of properties that the methods time out on when using a cut-off time of 100s. The best performing method for each subcategory is highlighted in bold.}
	\label{table:main_base}
\end{table}

==> Tables/old/debug.tex <==

% \subsection{Tables in process}
%  \sisetup{detect-weight=true,detect-inline-weight=math,detect-mode=true}
\begin{table*}[]

%% local settings
\sisetup{detect-weight,mode=text}
% for avoiding siunitx using bold extended
\renewrobustcmd{\bfseries}{\fontseries{b}\selectfont}
\renewrobustcmd{\boldmath}{}
% abbreviation
\newrobustcmd{\B}{\bfseries}

	\centering
	\scriptsize
	\setlength{\tabcolsep}{4pt}
	\aboverulesep = 0.1mm  % 0.605mm
	\belowrulesep = 0.2mm  % 0.984mm
	
	% bold elements in table
	%\renewrobustcmd{\bfseries}{\fontseries{b}\selectfont}
    %\renewrobustcmd{\boldmath}{}
    %\newrobustcmd{\B}{\bfseries}
    
	\begin{adjustbox}{center}

\begin{tabular}{lrrrrrr}
			& \multicolumn{2}{ c }{Base} & \multicolumn{2}{ c }{Wide} & \multicolumn{2}{ c }{Deep} \\
			\toprule

% \toprule
     Method &    Time(s) &  Timeout(\%) &  Time(s)\_wide &  Timeout(\%)\_wide &  Time(s)\_deep &  Timeout(\%)\_deep \\

    \cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
    
% \midrule
     AdvGNN &   0.521003 &    0.000000 &      0.855773 &         0.003300 &      2.081765 &         0.006667 \\
    MI-FGSM &   2.262002 &    0.005200 &      1.139254 &         0.003300 &      2.595880 &         0.008000 \\
 PGD Attack &  12.388920 &    0.071243 &      5.631557 &         0.024202 &      8.244899 &         0.032000 \\
\bottomrule
\end{tabular}

	\end{adjustbox}
	\caption{\small We compare average (mean) solving time, average number of subdomains solved, and the percentage of properties that the methods time out on when using a cut-off time of 100s. The best performing method for each subcategory is highlighted in bold.}
	\label{table:base_wide_deep}
\end{table*}




\begin{equation}

